Overparameterization Improves StyleGAN Inversion

Deep generative models like StyleGAN hold the promise of semantic image editing: modifying images by their content, rather than their pixel values. Unfortunately, working with arbitrary images requires inverting the StyleGAN generator, which has remained challenging so far. Existing inversion approaches obtain promising yet imperfect results, having to trade-off between reconstruction quality and downstream editability. To improve quality, these approaches must resort to various techniques that extend the model latent space after training. Taking a step back, we observe that these methods essentially all propose, in one way or another, to increase the number of free parameters. This suggests that inversion might be difficult because it is underconstrained. In this work, we address this directly and dramatically overparameterize the latent space, before training, with simple changes to the original StyleGAN architecture. Our overparameterization increases the available degrees of freedom, which in turn facilitates inversion. We show that this allows us to obtain near-perfect image reconstruction without the need for encoders nor for altering the latent space after training. Our approach also retains editability, which we demonstrate by realistically interpolating between images.

==> approach.tex <==
\section{Approach}




% While these experiments specifically address the optimization of network parameters, we find nothing \textit{per se} which would suggest a different behavior when optimizing for input parameters instead. Given these observations, we hypothethize that StyleGAN inversion would benefit from being less constrained. This can notably be accomplished by increasing the dimensionality of its input latent space, provided that we avoid degenerate conditioning (meaning, provided the the added dimensions are effectively used by the network). \\

% <!-- todo "constrained" comes out of nowhere -->

% Our work therefore answers the following two questions: 
% \begin{enumerate}
%     \item  Is inversion facilitated when StyleGAN's latent space is over-parameterized?
%     \item Will generation quality or editability be damaged when StyleGAN's latent space is over-parameterized?
% \end{enumerate}

==> experiments/colorization.tex <==

\newpage 

\begin{figure}[h]
    \includegraphics[width=\linewidth]{figures/inpainting.png}
    \caption{Denoising by invetering a blah blah.}\label{fig:colorization}
\end{figure}

\subsection{Colorization}

Denoising demonstrates the use of a stochastic loss function, and joint estimation of unknown parameters. Image shot noise is commonly modelled by a Poisson distribution, which converges to a Gaussian as $\sigma \rightarrow \infty$: 
\begin{equation}
\mathrm{poisson}(x; \sigma, \lambda) = \sigma 
\end{equation}
Our approach is inspired by noise2noise~\cite{noise2noise}. Given unknown parameters $(\sigma, \lambda)\in\mathcal{U}^2[0, 1]$, we set $f(x) = x + \xi $, where $\xi \sim \mathrm{poisson}(x; \hat\sigma, \hat\lambda)$ and $(\hat\sigma, \hat\lambda)$ are a jointly optimized estimators of the true parameters, initialized at 0. We then set $\lambda_{edit} = 0.2$ and $\lambda_{reg} = 0.05$. We hypothethise that our approach works as it both preserves \todo{blah blah sstatistics and makes fitting the noise harder}. 

% Following our overparmetrization, we are now able to constrain [[the latent vectors to the true input distribtion Z]]. Interestingly, we find that this constraint is insufficient to limit generation to produce realistic images [figure]. We remark that, while ,\\
% Noting that these [[atypical regions]] are limited to areas of low probability mass, we instead sample [[several points]] from the posterior distribution using Langevin Monte Carlo. 

\begin{table}[h]
\small
\begin{tabularx}{\linewidth}{Xcc}
\toprule
&\textbf{Fit [VGG] $\downarrow$}& \textbf{Realism [FID] $\downarrow$}\\
\midrule
Naïve Baseline & \_/\_ & \_/\_\\
PULSE (W+) & \_/\_ & \_/\_\\
Pivotal Tuning (W+) & \_/\_ & \_/\_\\
Our Approach & \_/\_ & \_/\_\\
\bottomrule
\end{tabularx}
\caption{Quality of the reconstruction (fit to the lowres target) and realism [[...]] of the distribution of upsampled images, measured on the AFHQv2 Cats test set.  }
\label{table:denoising_quality}
\end{table}

\begin{figure}[H]
    \includegraphics[width=\linewidth]{figures/singular_values.png}
    \caption{For any given image, our approach successfully recovers the true distribution parameters.}\label{fig:inpainting_robustness}
\end{figure}


==> experiments/deartifacting.tex <==

\newpage 


\begin{figure}[h]
    \includegraphics[width=\linewidth]{figures/inpainting.png}
    \caption{Inpainting the left part of an image by optimizing for the right part. Note that while the baseline also obtains realistic reconstruction, it is unable to do so without compromising fit quality. Our method is able to achieve both simultaneously.}\label{fig:inpainting}
\end{figure}


\subsection{JPEG Deartifacting}

JPEG deartifacting demonstrates the use of a differentiable approximation to a non-differentiable degradation process. 
JPEG compression is differentiable throughout\footnote{recall that JPEG compression consists of blah blah}, expect for the final quantization step, which rounds 

We use dsadsa's approximation to 


% Following our overparmetrization, we are now able to constrain [[the latent vectors to the true input distribtion Z]]. Interestingly, we find that this constraint is insufficient to limit generation to produce realistic images [figure]. We remark that, while ,\\
% Noting that these [[atypical regions]] are limited to areas of low probability mass, we instead sample [[several points]] from the posterior distribution using Langevin Monte Carlo. 

\begin{table}[h]
\small
\begin{tabularx}{\linewidth}{Xcc}
\toprule
&\textbf{Fit [VGG] $\downarrow$}& \textbf{Realism [FID] $\downarrow$}\\
\midrule
Baseline (W+) & \_/\_ & \_/\_\\
Baseline (Z) & \_/\_ & \_/\_\\
PULSE (W+) & \_/\_ & \_/\_\\
Pivotal Tuning (W+) & \_/\_ & \_/\_\\
Ours (Z, noise) & \_/\_ & \_/\_\\
\bottomrule
\end{tabularx}
\caption{Quality of the reconstruction (fit the of right part) and realism [[...]] of the distribution of inpainted images, measured on the AFHQv2 Cats test set for SGD/Adam. }
\label{table:inpainting_quality}
\end{table}

\begin{figure}[H]
    \includegraphics[width=\linewidth]{figures/singular_values.png}
    \caption{For any given image, our approach successfully recovers the true distribution parameters.}\label{fig:inpainting_robustness}
\end{figure}

==> experiments/denoising.tex <==

\newpage 

\begin{figure}[h]
    \includegraphics[width=\linewidth]{figures/inpainting.png}
    \caption{Denoising by invetering a blah blah.}\label{fig:denoising}
\end{figure}

\subsection{Denoising}

Denoising demonstrates the use of a stochastic loss function, and joint estimation of unknown parameters. Image shot noise is commonly modelled by a Poisson distribution, which converges to a Gaussian as $\sigma \rightarrow \infty$: 
\begin{equation}
\mathrm{poisson}(x; \sigma, \lambda) = \sigma 
\end{equation}
Our approach is inspired by noise2noise~\cite{noise2noise}. Given unknown parameters $(\sigma, \lambda)\in\mathcal{U}^2[0, 1]$, we set $f(x) = x + \xi $, where $\xi \sim \mathrm{poisson}(x; \hat\sigma, \hat\lambda)$ and $(\hat\sigma, \hat\lambda)$ are a jointly optimized estimators of the true parameters, initialized at 0. We then set $\lambda_{edit} = 0.2$ and $\lambda_{reg} = 0.05$. We hypothethise that our approach works as it both preserves \todo{blah blah sstatistics and makes fitting the noise harder}. 

% Following our overparmetrization, we are now able to constrain [[the latent vectors to the true input distribtion Z]]. Interestingly, we find that this constraint is insufficient to limit generation to produce realistic images [figure]. We remark that, while ,\\
% Noting that these [[atypical regions]] are limited to areas of low probability mass, we instead sample [[several points]] from the posterior distribution using Langevin Monte Carlo. 

\begin{table}[h]
\small
\begin{tabularx}{\linewidth}{Xcc}
\toprule
&\textbf{Fit [VGG] $\downarrow$}& \textbf{Realism [FID] $\downarrow$}\\
\midrule
Naïve Baseline & \_/\_ & \_/\_\\
PULSE (W+) & \_/\_ & \_/\_\\
Pivotal Tuning (W+) & \_/\_ & \_/\_\\
Our Approach & \_/\_ & \_/\_\\
\bottomrule
\end{tabularx}
\caption{Quality of the reconstruction (fit to the lowres target) and realism [[...]] of the distribution of upsampled images, measured on the AFHQv2 Cats test set.  }
\label{table:denoising_quality}
\end{table}

\begin{figure}[H]
    \includegraphics[width=\linewidth]{figures/singular_values.png}
    \caption{For any given image, our approach successfully recovers the true distribution parameters.}\label{fig:inpainting_robustness}
\end{figure}


==> experiments/encoding.tex <==
 
\subsection{Encoding Quality}
For our encoder, we use \textit{In-Domain GAN inversion} as our baseline, which, in our approach, we modify to output 512 vectors as previously described in section [method]. We set $\lambda_{discr}=0.2$ and train with a batch size of 4. While some approaches have investigated training the encoder jointly with the generator[][], we train the encoder separately as this approach is more commonly used in previous work (hence, this makes our results more comparable). Many papers specialize on human faces and improve results artificially by including a facial identity losses[][] (ArcFace[]). More recent approaches also attempt to generalize identity losses to other datasets[][][] (MoCo), but to avoid specializing our experiments we dispense of these losses altogether.\\
 \begin{figure}[H]
    \includegraphics[width=\linewidth]{figures/encoder_reconstruction.png}
    \caption{Selected reconstructions for our encoder trained on AFHQv2, with inlayed (VGG) reconstruction quality. Encoding quality is significantly improved when targeting an overparameterized latent space.}\label{fig:generation_quality}
\end{figure}
\noindent
We measure the perceptual (VGG) distance[] between the test set targets and reconstructions, and the FID between the distributions of reconstructions and the combined training and test set\footnote{This approach is typical[][] since the FID is a biased metric[] which is highly sensitive to the sample size.}. Our approach obtains much better reconstruction quality while maintaining a high level of realism, lending support to our hypothesis that StyleGAN inversion is overconstrained on the baseline's latent space.
\begin{table}[H]
\small
\centering
\begin{tabularx}{\linewidth}{Xcc}
\toprule
% Quality
&\textbf{ VGG (Distortion) $\downarrow$}& \textbf{FID (Realism) $\downarrow$}\\
\midrule
Baseline & \todo{--} & \todo{\textbf{--}} \\
Our method & \todo{\textbf{--}} & \todo{--}\\
\bottomrule
\end{tabularx}
\label{table:generation_quality_metrics}
\caption{VGG (reconstruction quality) and FID (realism) for the AFHQv2 datasets. }
\end{table}
\vspace{-2.00mm} 


\newpage


==> experiments/inpainting.tex <==

\newpage 

\begin{figure}[h]
    \includegraphics[width=\linewidth]{figures/inpainting.png}
    \caption{Inpainting the left part of an image by optimizing for the right part. Note that while the baseline also obtains realistic reconstruction, it is unable to do so without compromising fit quality. Our method is able to achieve both simultaneously.}\label{fig:inpainting}
\end{figure}

\subsection{Inpainting}

Inpainting is a common image restoration task, .

For this task, we define the degradation process as $f(x) = \mathrm{set the left half of x to 0}$, where we select the mask size from $\mathcal{U}[0, 1]$. 
We then set $\lambda_{edit} = 0.2$ and $\lambda_{reg} = 0.05$.

Note that, in many tasks, the , leading to specialized approaches which .
In contrast, our approach handles large masks despite not being specialized. 


\begin{figure}[H]
    \includegraphics[width=\linewidth]{figures/inpainting_robustness.png}
    \caption{When optimizing on the true input distribution Z, inpainting is robust even when the masked section covers the majority of the target image, or masks with highly unusual shapes.}\label{fig:inpainting_robustness}
\end{figure}

\begin{table}[h]
\small
\begin{tabularx}{\linewidth}{Xcc}
\toprule
&\textbf{Fit [VGG] $\downarrow$}& \textbf{Realism [FID] $\downarrow$}\\
\midrule
Naïve Baseline & \_/\_ & \_/\_\\
PULSE & \_/\_ & \_/\_\\
Pivotal Tuning & \_/\_ & \_/\_\\
Our approach & \_/\_ & \_/\_\\
\bottomrule
\end{tabularx}
\caption{Quality of the reconstruction (fit the of right part) and realism [[...]] of the distribution of inpainted images, measured on the AFHQv2 Cats test set for SGD/Adam. While the baseline must choose between good fit quality or realistic inpainting, ours is able to acheive both simulatenously.  }
\label{table:inpainting_quality}
\end{table}


==> experiments/joint.tex <==
\begin{table*}
\small
\begin{tabularx}{\linewidth}{Xcc}
\toprule
&\textbf{Fit [] $\downarrow$}& \textbf{Realism [FID] $\downarrow$}\\
\midrule
Naive Baseline & \_/\_ & \_/\_\\
PULSE & \_/\_ & \_/\_\\
Pivotal Tuning & \_/\_ & \_/\_\\
Ours & \_/\_ & \_/\_\\
\bottomrule
\end{tabularx}
\caption{Fit quality and prediction realism for various composed image restoration tasks. }
\label{table:composed}
\end{table*}

\newpage 

\subsection{Composed Image Restoration}
Our approach is particularly effective when the degradation can be understood as the composition of two or more separate functions, say, $f_1$ and $f_2$. Naive supervised approaches would learn two separate minimizers $g_{\theta_1}$ and $g_{\theta_2}$, trained separately to invert $f_1$ and $f_2$:
\vspace{2.5pt}
\begin{equation}
\argmin_{\theta_1} \mathbb{E}_{\mathbf{y}^*}\big[\mathcal{L}(g_{\theta_1}(\mathbf{y}_1), \mathbf{y}^*)\big] 
\end{equation}
\vspace{-10pt}
\begin{equation}
\argmin_{\theta_2} \mathbb{E}_{\mathbf{y}^*}\big[\mathcal{L}(g_{\theta_2}(\mathbf{y}_2), \mathbf{y}^*)\big] 
\end{equation}
Where $\mathcal{L}$ is an image distance metric\footnote{In practice the loss function would obviously vary between tasks, but for clarity we will assume it is the same for all of them.}, $g_{(\cdot)}$ is a parametric model, $\mathbf{y}^*$ are known, clean targets while $\mathbf{y}_1 = f_1(\mathbf{y}^*)$ and $\mathbf{y}_2 = f_2(\mathbf{y}^*)$ are the degraded targets\footnote{Some specialized approaches like Noise2Noise~\cite{noise2noise} can cleverly avoid the need for clean targets, but our approach never requires them.}. Naively composing these two models (Figure \ref{fig:failure_trained_composition}) leads to predictions of low quality, because the tasks are not independent:
\begin{equation}
\mathbb{E}_{\mathbf{y}^*}\big[\mathcal{L}(g_{\theta_1}(g_{\theta_2}(\mathbf{y})), \mathbf{y}^*)\big] \gg \min_\theta \mathbb{E}_{\mathbf{y}^*}\big[\mathcal{L}(g_\theta(\mathbf{y}), \mathbf{y}^*)\big]
\end{equation}
Where $\mathbf{y} = f_2(f_1(\mathbf{y}^*))$. \todo{Training for all sets of tasks is logistically difficult and impractical.} In contrast, we assume knowledge of $f_1$ and $f_2$ and instead parameterize a data prior using a generator-encoder pair $(G, E)_{\psi}$. In this way, we can directly solve for the image while accounting for the dependencies between all degradations:
\begin{equation}
\argmin_{\mathbf{x}\in G} \mathcal{L}(f_2(f_1(\mathbf{x})), \mathbf{y})
\end{equation}
Where we use the encoder $E$ to help constrain $\mathbf{x}$ to $G$'s output distribution. 
As compared to the naive approach, our method differs in that it does not require a clean target $\mathbf{y}^*$ and that it minimizes the loss over a single exemplar without training for any specific task.\\

\begin{figure}[H]
    \includegraphics[width=\linewidth]{figures/inpainting_robustness.png}
    \caption{Trained models \todo{(which ones)} which perform well on individual tasks fail when composed.}\label{fig:failure_trained_composition}
\end{figure}

\newpage 

\textbf{Protocol}\\
- Since trained approaches fail, we do not compare to them\\
- Note that, for most tasks, it is possible to infer an ordering over the functions \\
- we can only train or 2-3 tasks at once, otherwise we get poor quality 


==> experiments/restoration.tex <==
\section{Image Restoration}

Image restoration can be framed as finding an invert to a target $y$, after it has  degradation function [][]. 


\todo{quick intro, protocol, then explain which methods we are comparing against}   

==> experiments/style_mixing.tex <==
\subsection{Real Image Style Mixing}

\begin{figure}[H]
    \vspace{-4mm}
    \includegraphics[width=\linewidth]{figures/style_mixing.pdf}
    \caption{Style mixing on real (inverted) images. Our method can successfully transfer the style of the (real) right images onto the (real) bottom images, yielding the hybrid images in the middle.}\label{fig:style_mixing}
\end{figure}

We find that style mixing still works as expected with our revised style injection mechanism, which we briefly demonstrate on real (inverted) images. Our approach leaves the style mixing regularization unchanged, the only difference being that each layer is parameterized by up to 512 vectors rather than 1. In figure \ref{fig:style_mixing}, we mix the first 10 layers of the content image with the rest of layers for the style images, which matches the coloration and fine-detail of the style image while leaving the content intact.
\newpage
%  We might also want the baseline? The issue is that the cutoff point will have to change, and that the baseline might also be better :p 

% We could flesh this out with a table (FID) or sensitivity on each layer, also maybe a "slow" interpolation image showing each image 1 at a time. I'm not sure if this is a good idea...

==> todo.tex <==

- clarify our W w variables from the mathcal spaces. 

- supplemental for samples
- supplemental, more datasets
- supplemental for inversions
- supplemental for interpolations
